CoLadder: Supporting Programmers with Hierarchical Code Generation in Multi-Level Abstraction

Programmers increasingly rely on Large Language Models (LLMs) for code generation. However, misalignment between programmers' goals and generated code complicates the code evaluation process and demands frequent switching between prompt authoring and code evaluation. Yet, current LLM-driven code assistants lack sufficient scaffolding to help programmers format intentions from their overarching goals, a crucial step before translating these intentions into natural language prompts. To address this gap, we adopted an iterative design process to gain insights into programmers' strategies when using LLMs for programming. Building on our findings, we created CoLadder, a system that supports programmers by facilitating hierarchical task decomposition, direct code segment manipulation, and result evaluation during prompt authoring. A user study with 12 experienced programmers showed that CoLadder is effective in helping programmers externalize their problem-solving intentions flexibly, improving their ability to evaluate and modify code across various abstraction levels, from goal to final code implementation.

==> versions/v0.1/1_intro.tex <==
%%%%%% Major Contribution %%%%%%%
% V1: Support prompt authoring through matching between code and task structures (task decomposition, incremental generation, and multi-level abstraction) to help programmers validate code by reducing abstraction gaps. Provide controllability to scaffold to their desired level of abstraction

% V2: CodeXBlock provides interactive scaffolding from programming tasks to generated code, incorporating task decomposition, incremental generation, and multiple levels of abstraction to help programmers (not only) verify code during prompt authoring.



%%%%% TODO %%%%%%%%%
% Instead of spending that many paragraphs to talk about the verification, focus on the abstraction matching issue
% define the scope, not the software but the program (in RW)
% usage scenario - function, reuse...
% e.g., Jian writes some function
% add the focus point of "control loss" & "cognitive switching"
% controllability - Norman [33] and Höök [16] both recommended building safeguards like verification steps or controlling levels of autonomy to help prevent unwanted adaptations or actions from intelligent systems.
% serious harm when users cannot efectively understand or control an AI system (e.g., collaboration with semi-autonomous cars [41])

%%%%% SYNC words %%%%%%%%%
% programmers
% intention (contrast to expectation)
% LLM-based code assistants 



% ______________________________

\section{Introduction}


% LLM is growing
The advancement of Large Language Models (LLMs) \cite{chen2021evaluating, li2022competition} has led to significant progress in AI-driven code assistants \cite{Friedman_2021}.
% 
By leveraging the power of LLMs, these assistants have extended their functionality beyond code completion to generate sophisticated and high-quality code suggestions in response to natural language prompts \cite{bubeck2023sparks, nijkamp2022codegen, chen2021evaluating, chen2022codet, fried2022incoder}.
% advantage of LLM
% This transformation enables programmers to reduce the time spent on routine tasks \cite{sarkar2022like, barke2023grounded}, enhance productivity \cite{vaithilingam2022expectation, ziegler2022productivity}, and obtain guidance for unfamiliar problems \cite{barke2023grounded}.
% from copilot -> pilot (code assistants)
% These LLMs are capable of generating entire codebases with few lines of instructions \cite{Richards_2023},even shifting the role of code assistants from copilots to pilots in some programming processes.
Thanks to their ability to generate anywhere from a function of just a few lines of code to an entire codebase with just a few lines of instruction~\cite{Richards_2023}, LLLM-based code assistants are revolutionizing the way programmers reason, plan, and write code.
% from editing -> reviewing [A] (programmers)
% Consequently, programmers have redirected their primary focus from writing code to tasks such as crafting prompts and reviewing the code generated \cite{mozannar2022reading, bird2022taking}.


% issues of LLM
Despite their tremendous potential to make the programming process efficient by allowing programmers to delegate mundane tasks (e.g., code implementations) to AI and focus on high-level design (i.e., program logic), recent research into programmers' practices and experiences with code assistants revealed that new issues emerge and prevent programmers from achieving optimal efficiency. Specifically, researchers found that because AI instantly generates multiple lines of code for programmers --- which programmers cannot immediately get a sense of their validity and accuracy without reading them in detail, they often need to invest significant effort and cognitive load in verifying the AI-generated code \cite{tang2023empirical, vaithilingam2022expectation, sarkar2022like, xu2022ide, huang2023anpl}. 
% \fixme{They also find that programmers ... }
% \sangho{Perhaps mention several other challenges (beside the need to verify AI-generated code)? This paragraph can be just about new challenges that emerged from coding with AI asssitants and tthen in the next paragraph we can dive deeper into the challenges with the verification process?}
% why it's difficult
% several challenges emerge during the verification process. 
Instead of streamlining the programming process as imagined, the need to verify the AI-generated code can make the process rather cumbersome and pose additional cognitive load as programmers need to switch back and forth between code writing and code review, and edit the code when there is a misalignment between the AI-generated code and the programmer's intention \cite{chen2021evaluating}.

% such as dealing with cumbersome generated code, the additional cognitive load of switching back and forth between code writing and code review, and the misalignment between the AI-generated code and the programmer's intention \cite{chen2021evaluating}.
% alignment failure
% expectations.
% and iteratively refining the initial prompt \cite{mozannar2022reading, bird2022taking} to achieve the desired results.
% from the direction of code verifying
This \textit{alignment failure} exacerbates the challenges of verifying AI-generated code
% , which involves several strenuous steps such as comprehending the meaning of the code, evaluating its correctness and usefulness according to users' expectations, and verifying its integration with the existing codebase.
% This discrepancy makes verifying and comprehending AI-generated code become extremely difficult
because the mapping between natural language prompt and generated code is poorly understood \cite{liu2023wants}, which is referred to as \textit{abstraction matching issue} \cite{sarkar2022like}.
% (Mu & Sarkar, 2019; Luger & Sellen, 2016)
% which refers to the challenge of bridging the gap between the high-level abstractions conveyed through natural language and the precise implementation details required by the code.
% 
% Previous studies have shown that the mapping between natural language and code is poorly understood, that generated code can contain subtle bugs, and that generated code can be difficult to verify [95, 112, 124].
% % challenges
% from editing -> reviewing [A]
% One significant challenge arises from the shift in focus for programmers, as they have redirected their primary focus from writing code to tasks such as iteratively refining the prompt \cite{mozannar2022reading, bird2022taking} and verifying the code generated \cite{mozannar2022reading, bird2022taking}.
% This change has led programmers to invest substantial effort and time in verifying the AI-generated code \cite{tang2023empirical, vaithilingam2022expectation, sarkar2022like, xu2022ide, huang2023anpl}, as well as iteratively refining the initial prompt \cite{mozannar2022reading, bird2022taking} to achieve the desired results.
%% abstraction matching
% These challenges are intertwined with the issue of abstraction matching, which occurs when programmers must align their intentions and instructions with the capabilities of the system \cite{sarkar2022like}.
This is a long-discussed issue in most natural language interfaces, where programmers must align their intentions and instructions with the capabilities of the system \cite{}.
%% fuzzy abstraction matching
The abstraction matching issue becomes more `fuzzy' in the context of LLMs because of their inherent flexibility to generate plausible and correct results across different levels of abstraction \cite{sarkar2022like, chen2021evaluating}.
% LLMs exhibit the flexibility to generate plausible and correct results across various levels of abstraction.
While this flexibility allows users to immediately engage in prompting without careful thought and obtain usable results with minimal initial understanding, it makes it vulnerable to the abstraction matching issue.
% also provides a higher ceiling for achieving maximum productivity \cite{sarkar2022like}.
%
% Hence, programmers need to construct a cohesive mental model that effectively combines their understanding of different code assistants with the specific syntax requirements of the programming language \cite{liu2023wants}. 


% strategies to boost the verification process
To expedite the verification process, some programmers choose to quickly assess the code based on its `shape' \cite{barke2023grounded}, deferring verification by commenting out suggestions \cite{mozannar2022reading}, or even bypassing verification entirely \cite{barke2023grounded}.
% The importance of code comprehension [CITATION NEEDED]
While these approaches may provide a time-saving shortcut akin to opportunistic programming, it is essential to recognize the importance of code verification and program comprehension.
% problems if lack of comprehension
Insufficient comprehension can lead to misunderstandings \cite{maalej2014comprehension}, posing challenges for programmers when making code changes \cite{singer2010examination}, modifying the generated code, maintaining control over their program, and underestimating the effort required to debug \cite{vaithilingam2022expectation}.
% The utilization of LLM-based code assistants exacerbates these challenges, leading to difficulties for programmers in modifying the generated code and maintaining control over their program \cite{vaithilingam2022expectation}.
\ryan{Add Over-reliance literature here}
Based on prior research, it has been noted that when programmers postpone or skip the verification process, they tend to become overly dependent on the generated results and assume that they are always correct. This can lead to problems such as decreased task performance [3, 24], reduced trust [3, 56], and worsen user experience [28].
% 
% Hence, it is essential to alleviate the effort of verifying generated code, thereby lowering the issues of overreliance
% , which complements the work by Vasconcelos et al
% highlighting parts of generated code that might need human intervention.
% \cite{sarkar2022like, vaithilingam2022expectation}
% Previous work \cite{chen2021evaluating} explores numerous implications of AI models that generate code, including issues of over-reliance, and misalignment (the mismatch between what the user prompts requests and what the user wants). Over-reliance occurs when individuals make optimistic assumptions about the correctness of the output of an AI model, leading to harm
% overreliance on AI, which prior work has shown can decrease task performance [3, 24], reduce trust [3, 56], and worsen user experience [28].  -- Generation Probabilities Are Not Enough
%
% !!!! We need to provide them with controllability



%% from the direction of prompt engineering 
Previous research has proposed \textit{prompt engineering} \cite{strobelt2022interactive, liu2023pre} as a mitigation to address the issue of abstraction matching. These strategies encompass various techniques, such as introducing new programming languages \cite{huang2023anpl, beurer2023prompting}, automating prompt rewording, providing suggestions for simpler tasks, employing programming by demonstration techniques \cite{cypher1993watch, lieberman2001your}, and supporting task breakdowns \cite{ritschel2022can, liu2023wants}.
% examples
By breaking down complex problems into simpler sub-tasks, the gap in abstraction is reduced, enabling successful guidance of the model to execute the programmer's intentions \cite{bodker2015third}.
% This includes approaches such as introducing new programming languages \cite{huang2023anpl, beurer2023prompting}, automating prompt rewording, providing suggestions for simpler tasks, employing programming by demonstration techniques \cite{cypher1993watch, lieberman2001your}, and supporting task breakdowns \cite{ritschel2022can, liu2023wants}.
% used in many domains
% This approach is a common practice in program synthesis [2, 45], interactive dialogue systems [28, 68], and cognitive science [15, 25].
%
% difficulties in understanding the correct level
%too detail -> bad
However, determining the `correct' level of abstraction remains a challenge, as overly detailed prompt decomposition can result in the programming process with LLMs resembling the use of a ``highly inefficient programming language'' \cite{sarkar2022like}.
% the need of incremental guidance
Therefore, there is a need to provide programmers with guidance to gradually reveal the capabilities of these code assistants \cite{luger2016like}.
% By providing this scaffolding, programmers can effectively bridge the gap between their intentions and the generated code.




%% research goal -- [[need refined]]
The goal of this study is therefore to understand and explore design opportunities for programmers to effectively scaffold the abstraction gap between code and programming tasks.
% formative study reason
To understand what strategies and needs are for programmers to effectively overcome the issue of abstraction matching in the verification process, we conducted a formative study with six programmers who regularly use LLM-based code assistants.
% explore the strategies employed by programmers to mitigate challenges when using LLM-based code assistants and identify opportunities to improve the prompt authoring and code verification processes.
%% formative study 
% We identified a list of challenges when programmer verifying the AI-generated code, and strategies they employed.
% 
The formative study found that participants tend to
% prefer utilizing AI for smaller, simpler tasks, driven by their desire for understanding and control over their code. They 
decompose these tasks into sub-tasks and rely on their preconceived program structure and pseudocode syntax to guide the AI-generated code implementation.
% To meet specific requirements, participants may include code-level details in prompts and provide step-by-step guidance corresponding to the code structure.
Notably, participants relied on the code assistant's auto-completion prompts to verify that the generated code matched their intentions. They would wait for the complete prompt to be generated by assistants to ensure that the results were accurate. They would skip further detailed code verification because they believed that accurate prompt suggestions indicated that the LLM had effectively captured their intent.
% implications
% This highlights the potential of addressing the abstraction matching issue in the verification process through the prompt authoring process. By improving prompt construction and guiding LLMs to incrementally generate results at a lower level of abstraction, users can gain increased confidence in the generated code and reduce their reliance on extensive code verification.
%% Design Guidelines
These results highlighted the possibility to assist programmers in verifying the result by generating a lower abstraction level (e.g., from task to subtasks, from prompt to pseudocode), instead of directly generated the code.
% the need to provide programmers with step-by-step prompting and visual cues to help them navigate through the different levels of abstraction between the prompt and the code.
% potential strategies to alleviate these challenges. These include breaking down prompts into smaller, manageable blocks (D1); introducing multi-level of abstraction (D2) that utilizes a tree-based structure for prompt authoring; ensuring correspondence between code and prompt (D3) through visual cues; and incremental generation (D4), which involves generating code step by step to reduce the cognitive burden and allow for a gradual formation of the whole program.


%% system design
Informed by the formative study results, we propose \sys{}, a system that provides controlled scaffolding from programming tasks to generated code to help programmers verify code during the prompt authoring process.
%
\sys{} reducing the challenges to verify generated code by providing incremental generation, enabling a step-wise descent on the abstraction ladder from main tasks to sub-tasks, pseudocode, and ultimately actual code segments.
\sys{} allows programmers to gradually comprehend the generated code, verify it, and maintain control over the generation process while addressing the challenges inherent in prompt engineering and code verification.
% \sys{} strengthens the connection between the programmers' mental model, the prompt, and the generated code, reducing the cognitive burden of verifying generated code.
%% iterative design process
We iteratively designed the system and conducted a cognitive walkthrough with six experienced programmers to pinpoint features needed for their prompt-based programming authoring process. 
%% features
% \sys{} employs a block-based text editor and a tree-based prompt structure to assist the prompt authoring process. 
%% Evaluation
To evaluate the utility of \sys{} by conducting an evaluation study with 12 experienced programmers who frequently use LLM-based code assistants.
\ryan{Why experienced programmers}
% Considering that previous studies suggest that code generation quality depends on user experience level [98], that less experienced users had difculty understanding, editing, and debugging generated code [84] - On the Design of AI-powered Code Assistants for Notebooks

% The results demonstrated that our system effectively addresses the identified challenges, enriches the prompt-based programming authoring process, and provides an interactive environment for incremental code generation.

%%% Contributions
% This research thus contributes in three folds: It unveils the challenges programmers face while working with AI-generated code, proposes a novel system design to address these challenges, and provides empirical evidence of the system's efficacy through an expert evaluation.

In summary, we contribute:

\begin{itemize}
    \item \sys{}, a system that demonstrates the notion of controlled scaffolding from programming tasks to generated code, to help programmers verify code during the prompt authoring process; 
    \item A user study demonstrating and 
    \item 
\end{itemize}


% -> how to let programmer reading the code while prompting



% NEED - code modification issue
% NEED - how do we solve the code verification issue



% Previous research has highlighted that developers spent the most time on the stage of ``thinking and verifying the suggestions,'' indicating that verification is a crucial aspect of AI-assisted programming. Additionally, incorrect code generated by AI-assisted programming tools can lead to a time-consuming debugging rabbit hole, which can hinder the completion of programming tasks. Furthermore, prompting modifications to the generated code can be challenging, especially if the modifications require significant changes to the original source code. These findings indicate that the AI-assisted programming tools has shifted the programming task for developers from coding to code reviewing, and the importance of assisting developers in verifying and modifying generated code. While previous research has developed tools that can help prompt engineers reduce the abstraction gap between natural language prompts and the generated content by providing visualizations to the prompts, there is also a need to apply visualizations to programs and code to improve programmer comprehension and reduce the burden of code modification.


% Significant research has attempted to reduce the cognitive burden for the programmer on understanding code through the program visualizations, which can be categorized into three levels: software visualization, program visualization, and code visualization. In recent years, node-based code editors have gained widespread popularity as visual programming methods due to their intuitive and interactive nature. Instead of writing traditional text-based code, programmers can construct programs by connecting nodes that represent different functionalities or operations. Several open source projects have leveraged node-based editor to build LLM-based software, or integrated AI to node-based code editor for developers to accomplish the desired functions without directly interacting with the source code. This integration allows programmers to express their intent through natural language prompts, which the LLM interprets and converts into executable code represented by nodes. The utilization of LLM-powered node-based code editors brings notable benefits, encompassing heightened code comprehension, enhanced programming efficiency, and the provision of a no-code experience that proves particularly advantageous for novice programmers or individuals lacking coding expertise. Despite the assistance provided by these tools in expediting effortless and efficient software development, it remains crucial for experienced developers to possess a sufficient understanding of their own source code, which empowers them to effectively navigate, maintain, modify, debug, and optimize the software, ensuring its long-term viability. However, while using AI-assisted programming tools, developers have observed a loss of control over their programs, which may lead to the debugging and maintaining the code becoming difficult over time. As a result, it is critical to implement program or code-level visualizations to assist developers in understanding and interacting with the code generated by LLM.


% Our objective is thus to design and implement program visualizations at multiple levels of abstraction, empowering developers to effortlessly comprehend the code generated by AI. And we aim to provide interaction design that seamlessly integrate natural language prompts, allowing developers to modify the code by interacting with the visual elements with ease and precision. To achieve this goal, we conducted a formative study to gain insights into how users verify and utilize AI-generated code, as well as their approach to modifying the code through re-prompting. This study encompassed various aspects, including how users specify the location to make changes, how they verify and assess the newly generated code, and how they integrate the modified code into their programs. By understanding these user behaviours and preferences, we can derive valuable insights that inform the design of effective program-level visualizations. The findings from our formative study shed light on several key aspects.
% % TODO: What are the findings from the formative study, e.g., Firstly... These insights highlight the importance of providing visual cues and feedback to aid in the verification and modification process.


% Leveraging the design guidelines established by previous research on program visualization and the insights derived from our formative study, we developed \sys{}, a novel system that combines program-level visualization techniques with AI-generated code to facilitate code comprehension and modification. 
% TODO: what \sys{} can do...


% To evaluate...
% TODO evaluation and major findings


% Our contribution is in three-folds...
% TODO: Main contributions



% Software visualization provides an overview of the program structure and its interactions with external systems. Program visualization shows how the program is organized and the relationships between its components. The code visualization displays the source code in a readable and understandable format.




% Finally, LLMs can also be a source of frustration for developers who feel like they are losing control over their programs. While LLMs can be powerful tools for generating code, they can also be unpredictable and difficult to understand, which can make it harder for developers to debug and maintain their code in the long term.

==> versions/v0.1/2_rw.tex <==
\section{Background and Related Work}

\subsection{Programmer-LLM Interaction}
% AI-powered programming assistant 
% introduce LLM-based programming assistants
% How programmers using LLM-based programming assistants
The interaction between programmers and AI has been explored in a variety of ways, while our focus is on deep learning model-driven code generation tools. These models exhibit the capability to produce code based on plain language explanations or incomplete code snippets after being trained on a large amount of existing codebase \cite{kite_2014, balog2016deepcoder, hayati2018retrieval, jiang2021treebert, tabnine, yin2017syntactic}
% 
Recent advances in LLMs, exemplified by GPT-4, LLaMa, and PaLM 2, mark a significant breakthrough in code generation compared to preceding deep-learning models.
% 
Studies have shown that the accuracy of code assistants has improved significantly \cite{chen2021evaluating, pearce2023examining}, thereby enriching user experience, and increasing perceived productivity \cite{ziegler2022productivity, li2022competition, vaithilingam2022expectation}, especially in tasks that involve repetition \cite{sarkar2022like, barke2023grounded}.


\paragraph{\textbf{Challenges of Verification}}
However, programmers dedicate considerable time to validating AI-generated suggestions \cite{mozannar2022reading, barke2023grounded}.
% Understanding the Usability of AI Programming Assistants
Liang et al. \cite{liang2023understanding} conducted a survey study highlighting that current code generation tools face several usability challenges, including difficulties in comprehending the relationship between the programmer's prompt and the following generated code, as well as struggles in guiding these models to achieve desired outputs.
% grounded copilot
Barke et al. \cite{barke2023grounded} elaborate strategies programmers employ to accelerate the verification process when using code generation tools. These strategies include accepting suggestions without validation, deferring the validation process, or using code as the prompt rather than natural language. The findings also noted that programmers sometimes validate generated code based on keywords and explanations, which aligns with previous eye-tracking research on understanding code readability issues and visual inspections of generated code \cite{al2022readable}.
% Expectation v.s. Experience
Vaithilingam et al. \cite{vaithilingam2022expectation} report that programmers using LLM-based code assistants often fail to complete their programming tasks. This problem occurs due to an underestimation of the time required to align the generated code with the programmer's intent, which often leads to debugging rabbit hole. They conclude with the need to support programmers in verifying generated code and to empower them with more control over the code for subsequent editing, debugging, and maintenance.

\paragraph{\textbf{Abstraction Matching Issue}}
% abstraction matching - what is it like
Sarkar et al. \cite{sarkar2022like} highlight the difficulty of abstract matching in the verification process, where programmers need to conceptualize the boundaries of model abilities and the required naturalistic utterances to maximize productivity. This issue is rooted in the notion of the \textit{gulf of execution} \cite{hutchins1985direct}, about challenges in translating user instructions into executable computer tasks. The problem of matching abstractions becomes more noticeable due to the LLMs' capability to create code at different levels of abstraction, which consist of innumerable combinations of natural language expressions.
% 
Prior research into natural language interfaces suggests the benefit of managing expectations and gradually revealing the capabilities of the system through user interaction and intervention \cite{luger2016like, liu2023wants, ross2023programmer, vasconcelos2023generation}.
% other issues
Excessive validation overhead can lead to several issues \cite{vasconcelos2023generation, weisz2021perfection, ross2023programmer}. These include over-reliance on generated suggestions without verifying them \cite{barke2023grounded, chen2021evaluating, xu2022ide}, loss of control over their own programs when bypassing the verification step \cite{vaithilingam2022expectation}, which then introduces challenges when modifying the generated code \cite{vaithilingam2022expectation, cai2023low, al2022readable}, and the cognitive load of switching between programming and debugging tasks \cite{vaithilingam2022expectation, ferdowsi2023live, bastola2023llm, ma2023demonstration}


% Conclusion on Challenges
Based on previous research, we identified four major challenges for our work to address: \textbf{C1: }Misalignment between the LLM-generated code and the programmer's intent; \textbf{C2: }Loss of control over programmers' own code; \textbf{C3: }Over-reliance on code suggestions without verification; \textbf{C4: }Disruptive context switching between programming and debugging.

% \subsubsection{Abstraction Gap \& Control Loss}
% abstraction matching issue
% control loss issue
    % in different Human-AI domains as well
    % the need for verification


% \subsection{Human-AI Collaboration in Programming}
% controllability - Norman [33] and Höök [16] both recommended building safeguards like verification steps or controlling levels of autonomy to help prevent unwanted adaptations or actions from intelligent systems.

\subsection{Improving LLM-based Code Generation}
% current strategies to overcome these issues
    % technical strategies - training
    % new programming language
    % prompt engineering
    % interaction paradigm 
% but deciding the level of controllability remains a challenge

% “experienced programmers are willing to interact with code generation tools by rewriting problem descriptions in natural language [12].” (Conversing with Copilot: Exploring Prompt Engineering for Solving CS1 Problems Using Natural Language)

% When prompt engineering was required, modifications that resembled pseudocode tended to be the most successful - Conversing with Copilot

% Natural language-guided programming
% Pre-train, prompt, and predict: A systematic survey of prompting methods in natural language processin
% Prompt programming for large language models: Beyond the few-shot paradigm.
% Productivity Assessment of Neural Code Completion



\subsection{Visual Programming and Program Visualization}
% We refer to the design choice from the previous visual programming literature to support programmers in scaffolding their mindset to code.

% However, compared to these visual programming tools that usually targeted novice programmers, our tools focused on non-novice programmers. Because our tools mainly focused on "matching" instead of just "prompt decomposition", which required programmers have expectations of the code while writing the prompt and understand the code structure to verify the code.

